High-dimensional multidisciplinary design optimization for aircraft eco-design / Optimisation multi-disciplinaire en grande dimension pour l'\'eco-conception avion en avant-projet

The objective of this Philosophiae Doctor (Ph.D) thesis is to propose an efficient approach for optimizing a multidisciplinary black-box model when the optimization problem is constrained and involves a large number of mixed integer design variables (typically 100 variables). The targeted optimization approach, called EGO, is based on a sequential enrichment of an adaptive surrogate model and, in this context, GP surrogate models are one of the most widely used in engineering problems to approximate time-consuming high fidelity models. EGO is a heuristic BO method that performs well in terms of solution quality. However, like any other global optimization method, EGO suffers from the curse of dimensionality, meaning that its performance is satisfactory on lower dimensional problems, but deteriorates as the dimensionality of the optimization search space increases. For realistic aircraft design problems, the typical size of the design variables can even exceed 100 and, thus, trying to solve directly the problems using EGO is ruled out. The latter is especially true when the problems involve both continuous and categorical variables increasing even more the size of the search space. In this Ph.D thesis, effective parameterization tools are investigated, including techniques like partial least squares regression, to significantly reduce the number of design variables. Additionally, Bayesian optimization is adapted to handle discrete variables and high-dimensional spaces in order to reduce the number of evaluations when optimizing innovative aircraft concepts such as the "DRAGON" hybrid airplane to reduce their climate impact.

==> chapter1.5-Litterature/chapter2-literature.tex <==
\chapter{Chapter Title} 
\section{Review of Literature}
A literature review is a text of a scholarly paper, which includes the current knowledge including substantive findings, as well as theoretical and methodological contributions to a particular topic. Literature reviews are secondary sources, and do not report new or original experimental work. Most often associated with academic-oriented literature, such reviews are found in academic journals, and are not to be confused with book reviews that may also appear in the same publication. Literature reviews are a basis for research in nearly every academic field \citep{maedche2001ontology}. A narrow-scope literature review may be included as part of a peer-reviewed journal article presenting new research, serving to situate the current study within the body of the relevant literature and to provide context for the reader. In such a case, the review usually precedes the methodology and results sections of the work.

Producing a literature review may also be part of graduate and post-graduate student work, including in the preparation of a thesis, dissertation, or a journal article. Literature reviews are also common in a research proposal or prospectus (the document that is approved before a student formally begins a dissertation or thesis) \citep{doan2002learning, duzdevich2014dna}.

\section{Review Types}
The main types of literature reviews are: evaluative, exploratory, and instrumental \citep{duzdevich2014dna, thiruganam2010automatic}.

A fourth type, the systematic review, is often classified separately, but is essentially a literature review focused on a research question, trying to identify, appraise, select and synthesize all high-quality research evidence and arguments relevant to that question. A meta-analysis is typically a systematic review using statistical methods to effectively combine the data used on all selected studies to produce a more reliable result.


\subsection{Process And Product}
\cite{gilbarg2015elliptic} distinguish between the process of reviewing the literature and a finished work or product known as a literature review. The process of reviewing the literature is often ongoing and informs many aspects of the empirical research project. All of the latest literature should inform a research project. Scholars need to be scanning the literature long after a formal literature review product appears to be completed.

\section{Page Limitation}
A careful literature review is usually 15 to 30 pages and could be longer. The process of reviewing the literature requires different kinds of activities and ways of thinking \citep{duzdevich2014dna} and \cite{kothari2004research} link the activities of doing a literature review with Benjamin Bloom’s revised taxonomy of the cognitive domain (ways of thinking: remembering, understanding, applying, analysing, evaluating, and creating).

==> figs/archi.tex <==
\tikzstyle{abstract}=[rectangle, draw=black, rounded corners, anchor=north]
\tikzstyle{myarrow}=[->, >=open triangle 90, thick]
\tikzstyle{line}=[-, thick]

\begin{tikzpicture}[node distance=1cm, thick, scale=0.6, every node/.style={scale=0.8}]
\node (SMT) [abstract, rectangle split, rectangle split parts=2,text width=3.8cm,rectangle split part fill={blue!50,blue!10}]
{\textbf{SMT}
\nodepart{second}+ problems\\ + sampling\_methods\\ + surrogate\_models};
\node (AuxNode01) [text width=4cm, right=of SMT] {};
\node (problems) [abstract, rectangle split, rectangle split parts=2, below=of SMT,text width=2.7cm,rectangle split part fill={blue!50,blue!10}] {\textbf{problems::\\Problem}
\nodepart{second}+ \_\_call\_\_()\\\# \_evaluate()};
\node (sampling) [abstract, rectangle split, rectangle split parts=2, left=of problems,text width=4.15cm,rectangle split part fill={blue!50,blue!10}]
{\textbf{sampling\_methods::\\SamplingMethod}
\nodepart{second}+ \_\_call\_\_()\\\# \_compute()};
\node (surrogate) [abstract, rectangle split, rectangle split parts=2, below=of AuxNode01,text width=5.7cm,rectangle split part fill={blue!50,blue!10}]
{\textbf{surrogate\_models::\\SurrogateModel}
\nodepart{second}+ set\_training\_values()\\+ update\_training\_values()\\+ set\_training\_derivatives()\\+ update\_training\_derivatives()\\+ predict\_derivatives()\\+ predict\_output\_derivatives()\\+ predict\_variances()\\+ predict\_values()\\+ train()\\\# \_predict\_derivatives()\\\# \_predict\_output\_derivatives()\\\# \_predict\_values()\\\# \_predict\_variances()\\\# \_train()};
\draw[myarrow] (SMT) -| (sampling.north);
\draw[myarrow] (SMT) -- (problems.north);
\draw[myarrow] (SMT) -| (surrogate.north);
\end{tikzpicture}


==> figs/mlp_slides.tex <==
\begin{tikzpicture}

% N:node, 1:layer, (u,c,b) : up, center, below

% input-layer (first layer) %
\node [draw, circle, minimum size=0.75cm] (N1c) at (0,0) {\large $\alpha_i^{(in)}$};
\node [draw, circle, minimum size=0.75cm, xshift=0cm, yshift=3cm, at=(N1c), label={\hspace{-0.5cm} \vspace{0.5cm}  \large Input layer}] (N1u) {\large $\alpha_1^{(in)}$};
\node [draw, circle, minimum size=0.75cm, xshift=0cm, yshift=-3cm, at=(N1c)] (N1b) {\large $\alpha_p^{(in)}$};

\node [at=($(N1c)!0.5!(N1b)$)] {\Huge \vdots} ;
\node [at=($(N1c)!0.5!(N1u)$)] {\Huge \vdots} ;
%----------%


% 2nd layer %
%\node [draw, circle, minimum size=1cm, at=($(N1c)+(2.5,0)$)] (N2c) {};
%\node [draw, circle, minimum size=1cm, at=($(N1u)+(2.5,-1)$)] (N2u) {};
%\node [draw, circle, minimum size=1cm, at=($(N1b)+(2.5,+1)$)] (N2b) {};

\node [draw, circle, minimum size=0.75cm, xshift=3.5cm, yshift=0cm, at=(N1c)] (N2c) {};
\node [draw, circle, minimum size=0.75cm, xshift=0cm, yshift=3cm, at=(N2c)] (N2u) {};
\node [draw, circle, minimum size=0.75cm, xshift=0cm, yshift=-3cm, at=(N2c)] (N2b) {};

\node [at=($(N2c)!0.5!(N2b)$)] {\Huge \vdots} ;
\node [at=($(N2c)!0.5!(N2u)$)] {\Huge \vdots} ;
%----------%

% 3rd layer %
\node [draw, circle, minimum size=0.75cm, xshift=2.5cm, yshift=0cm, at=(N2c)] (N3c) {};
\node [draw, circle, minimum size=0.75cm, xshift=0cm, yshift=3cm, at=(N3c)] (N3u) {};
\node [draw, circle, minimum size=0.75cm, xshift=0cm, yshift=-3cm, at=(N3c)] (N3b) {};


\node [at=($(N3c)!0.5!(N3b)$)] {\Huge \vdots} ;
\node [at=($(N3c)!0.5!(N3u)$)] {\Huge \vdots} ;
%----------%


% 4th layer %
\node [draw, circle, minimum size=0.75cm, xshift=2.5cm, yshift=0cm, at=(N3c)] (N4c) {};
\node [draw, circle, minimum size=0.75cm, xshift=0cm, yshift=3cm, at=(N4c)] (N4u) {};
\node [draw, circle, minimum size=0.75cm, xshift=0cm, yshift=-3cm, at=(N4c)] (N4b) {};


\node [at=($(N4c)!0.5!(N4b)$)] {\Huge \vdots} ;
\node [at=($(N4c)!0.5!(N4u)$)] {\Huge \vdots} ;
%----------%



% % n-1 layer %
% \node [draw, circle, minimum size=0.75cm, xshift=5cm, yshift=0cm, at=(N3c)] (N6c) {}; %computed from N3c
% % boxed

% \node [draw, circle, minimum size=0.75cm, xshift=0cm, yshift=3cm, at=(N6c)] (N6u) {};

% \node [draw, circle, minimum size=0.75cm, xshift=0cm, yshift=-3cm, at=(N6c)] (N6b) {};

% \node [at=($(N6c)!0.5!(N6b)$)] {\Huge \vdots} ;
% \node [at=($(N6c)!0.5!(N6u)$)] {\Huge \vdots} ;
%----------%



% n layer %
\node [draw, circle, minimum size=0.75cm, xshift=0cm, yshift=0cm, at=(N4c)] (N7c) {}; 
\node [draw,  circle, minimum size=0.75cm, xshift=0cm, yshift=3cm, at=(N4c)] (N7u) {};
\node [draw, circle, minimum size=0.75cm, xshift=0cm, yshift=-3cm, at=(N4c)] (N7b) {};

% % Three nodes
% \node [at=($(N7c)!0.43!(N7b)$)] {\Huge \vdots} ;
% \node [at=($(N7c)!0.57!(N7u)$)] {\Huge \vdots} ;

% Two nodes
%\node [at=($(N7u)!0.42!(N7b)$)] {\Huge \vdots} ;
%----------%


% output  %
\node [draw, circle, minimum size=1cm, xshift=3cm, yshift=0cm, at=(N7c), label={ \large Output}] (N8c) {\large $\psi \left(\alpha^{(in)}\right )$}; %computed from N3c

\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N7c)--(N8c);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N7u)--(N8c);
\draw[ -{Stealth[length=2mm, width=1.5mm]}] (N7b)--(N8c);
%----------%

% % First fake layer
% \node [ circle, minimum size=0.75cm, at=($(N3c)!.33!(N6c)$)] (N4c) {};
% \node [ circle, minimum size=0.75cm, at=($(N3u)!.33!(N6u)$)] (N4u) {};
% \node [ circle, minimum size=0.75cm, at=($(N3b)!.33!(N6b)$)] (N4b) {};

% %% 2nd fake%%%
% \node [ circle, minimum size=1cm, at=($(N3c)!.66!(N6c)$)] (N5c) {}; 
% \node [ circle, minimum size=1cm, at=($(N3u)!.66!(N6u)$)] (N5u) {};
% \node [ circle, minimum size=1cm, at=($(N3b)!.66!(N6b)$)] (N5b) {};





%------------------------arretes ---------------------%

% input-to-2nd %
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N1c)--(N2c);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N1c)--(N2u);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N1c)--(N2b);

\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N1u)--(N2c);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N1u)--(N2u);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N1u)--(N2b);

\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N1b)--(N2c);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N1b)--(N2u);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N1b)--(N2b);
%----------%


% 2nd-to-3rd %
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2c)--(N3c);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2c)--(N3u);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2c)--(N3b);

\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2u)--(N3c);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2u)--(N3u);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2u)--(N3b);

\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2b)--(N3c);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2b)--(N3u);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2b)--(N3b);
% %----------%

% 3rd-to-4th %
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N3c)--(N4c);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N3c)--(N4u);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N3c)--(N4b);

\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N3u)--(N4c);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N3u)--(N4u);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N3u)--(N4b);

\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N3b)--(N4c);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N3b)--(N4u);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N3b)--(N4b);
% %----------%



% % between 3rd layer and 1st fake
% \draw[ - ] (N3c) -- ($(N3c)!.66!(N4c)$); %longer
% \draw[ - ] (N3c) -- ($(N3c)!.33!(N4u)$);
% \draw[ - ] (N3c) -- ($(N3c)!.33!(N4b)$);

% \draw[ - ] (N3u)-- ($(N3u)!.33!(N4c)$);
% \draw[ - ] (N3u)-- ($(N3u)!.66!(N4u)$); %longer
% \draw[ - ] (N3u)-- ($(N3u)!.25!(N4b)$); % shorter

% \draw[ - ] (N3b)-- ($(N3b)!.33!(N4c)$);
% \draw[ - ] (N3b)-- ($(N3b)!.25!(N4u)$); %shorter
% \draw[ - ] (N3b)-- ($(N3b)!.66!(N4b)$); %longer
% %------------------------%

% % between 1st-fake and 2nd-fake
% \node [at=($(N4c)!0.5!(N5c)$)] {\large \dots } ;
% \node [at=($(N4u)!0.5!(N5u)$), rotate=160] {\large \dots } ;
% \node [at=($(N4b)!0.5!(N5b)$), rotate=20] {\large \dots } ;
% %-----------------%

% % between 2nd-fake and n-1
% \draw[ -{Stealth[length=2mm, width=1.5mm]}  ] ($(N5c)!.5!(N6c)$)--(N6c); 
% \draw[ -{Stealth[length=2mm, width=1.5mm]}  ] ($(N5c)!.66!(N6u)$)--(N6u);
% \draw[ -{Stealth[length=2mm, width=1.5mm]}  ] ($(N5c)!.66!(N6b)$)--(N6b);

% \draw[ -{Stealth[length=2mm, width=1.5mm]}  ] ($(N5u)!.75!(N6c)$)--(N6c);
% \draw[ -{Stealth[length=2mm, width=1.5mm]}  ] ($(N5u)!.5!(N6u)$)--(N6u); 
% \draw[ -{Stealth[length=2mm, width=1.5mm]}  ] ($(N5u)!.8!(N6b)$)--(N6b); % fix

% \draw[ -{Stealth[length=2mm, width=1.5mm]}  ] ($(N5b)!.75!(N6c)$)--(N6c);
% \draw[ -{Stealth[length=2mm, width=1.5mm]}  ] ($(N5b)!.8!(N6u)$)--(N6u); % fix
% \draw[ -{Stealth[length=2mm, width=1.5mm]}  ] ($(N5b)!.5!(N6b)$)--(N6b); 
% %----------------%


% (n-1)-to-(n) %
% \draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2c)--(N7c);
% \draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2c)--(N7u);
% \draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2c)--(N7b);

% \draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2u)--(N7c);
% \draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2u)--(N7u);
% \draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2u)--(N7b);

% \draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2b)--(N7c);
% \draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2b)--(N7u);
% \draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2b)--(N7b);
%----------%



%-------------------------------------%
% Trapeze : 4 nodes connected
\node [circle, minimum size=1cm] (T1u) at ($(N2u)-(0.8,-0.8)$)  {};
\node [circle, minimum size=1cm] (T1b) at ($(N2b)-(0.8,0.8)$)  {};
\node [circle, minimum size=1cm] (T2u) at ($(N7u)+(0.8,0.8)$)  {};
\node [circle, minimum size=1cm] (T2b) at ($(N7b)+(0.8,-0.8)$)  {};
% left
\draw[dotted, line width= 0.4mm] ($(T1u)+(0,0)$)--($(T1b)+(0,0)$);
% right
\draw[dotted, line width= 0.4mm] ($(T2u)+(0,0)$)--($(T2b)+(0,0)$);

% upper
%\getangle(T1u)(T2u)a;
\draw[dotted, line width= 0.4mm] ($(T1u)+(0,0)$)--($(T2u)+(0,0)$) node[midway, above, black, %rotate=\anglea
]{\large $l=3$ hidden layers } ;

% lower
\draw[dotted, line width= 0.4mm] ($(T1b)+(0,0)$)--($(T2b)+(0,0)$);
%-------------------------------------%




% %curly brack for units in a layer
% \draw [decorate, decoration = {calligraphic brace,raise=15pt, mirror, amplitude=14pt}, line width = 0.4mm ] ($(N6u)-(0.5,-0.6)$) --  ($(N6b)-(0.5,0.6)$); 

% %
% \draw[->] ($(N5c)+(0,0)$) -- (7.5, -5) node[inner sep=8pt, at end, yshift=-0.5cm] {\Large $n_{l-1}$} ;


% % Boxed
% \node [draw, minimum size=0.85cm, line width=0.5mm, at=(N7u)] (N7U) {};

% \node [draw, minimum height=4.5cm, minimum width=12.5cm, xshift=2.5cm, yshift=6cm, line width=0.3mm, at=(N7U)] (box) {}; %%%%%%%

% \draw[->, inner sep=5pt] (N7U.north) .. controls +(down:0cm) and +(right:0cm) .. (box.south);

% \node (boxC) [draw, circle, minimum size=0.85cm, at=(box.west), xshift=2.5cm] {$\alpha_{2}^{(l-1)}$}  ;

% \node (boxCC) [ minimum size=0.85cm, at=(box.west), xshift=0.75cm] {\Large$n_{l-1}$}  ;

% \node (boxT) [draw, circle, minimum size=0.85cm, at=(boxC), yshift=1.5cm] {$\alpha_{1}^{(l-1)}$}  ;
% \node (boxB) [ circle, minimum size=0.85cm, at=(boxC), yshift=-1.5cm] { \vspace{-1cm} \Large \vdots }  ;
% \draw [decorate, decoration = {calligraphic brace,raise=15pt, mirror, amplitude=14pt}, line width = 0.4mm ] ($(boxT)-(0.2,-0.6)$) --  ($(boxB)-(0.2,0.6)$) ;

%\node (boxScal) [draw, minimum size=0.85cm, at=(boxC), xshift=3.25cm, label={Scalar product}] {$w^{\top} \cdot \alpha^{(l-1)}$}  ;

% \node (boxScal) [draw, minimum size=0.85cm, at=(boxC), xshift=3.25cm, label={Scalar product}] { 
% $   \sum \limits_{i=1}^{n_{l-1}} w_i \alpha_i^{(l-1)} $
% }  ;

% \draw[->] (boxT) -- (boxScal) node[midway, above, black]{$w_{1}$};
% \draw[->] (boxC) -- (boxScal) node[midway, above, black]{$w_{2}$};



% %---Activation func---%
% %label={Act. function}
% \node (boxAct) [draw, minimum size=0.85cm, at=(boxScal), xshift=3.25cm, label={Activation function}] {
% \begin{tikzpicture}
%         \begin{axis}[axis lines=center, width=3.5cm, axis x line shift=1cm, height=3.5cm,
%          yticklabels={,,},
%          xticklabels={,,}
%          ]
%         \addplot[color=black]{1/(1+exp(-x))-2};
%         \end{axis}
%         \end{tikzpicture}
% }  ;
% %------%

% \draw [->] (boxScal) -- (boxAct);

% \node (nodeRed) [draw, circle, minimum size=0.85cm, fill=black!25, at=(boxAct), xshift=2.5cm] {$\alpha_{1}^{(l)}$};

% \draw [->] (boxAct) -- (nodeRed);



\end{tikzpicture}

==> figs/variable_roles.tex <==
\begin{tikzpicture}
\node(1)[label={}, draw, circle]
at (0,0) 
{\begin{tabular}{c}
Meta (dimensional) \\
Component \\
$x_{\meta}$
\end{tabular}}  ;

\node(2)[label={}, xshift=-5cm, yshift=-1.5cm, at=(1), draw, circle]
{\begin{tabular}{c}
Neutral \\
Component \\
$x_{\neutral}$
\end{tabular}
}
;


\node(3)[label={Decreed}, circle, xshift=5cm, yshift=-2cm, at=(1), draw]
{\begin{tabular}{cc}
  Included  &    Excluded \\
  component &    component \\
  $x_{\decreed}$ &   $\overline{x_{\decreed}}$
\end{tabular}
};

\draw[dotted, line width=0.5mm] (5,0.6)--(5,-4.6);

\draw[->] (1)--(3);


\end{tikzpicture}
